Dirichlet-Neumann Waveform Relaxation Algorithm for Time Fractional Diffusion Equation in Heterogeneous Media

In this article, we have studied the convergence behavior of the Dirichlet-Neumann waveform relaxation algorithms for time-fractional sub-diffusion and diffusion wave equations in 1D \& 2D for regular domains, where the dimensionless diffusion coefficient takes different constant values in different subdomains. From numerical experiments, we first capture the optimal relaxation parameters. Using these optimal relaxation parameters, our analysis estimates the rate of change of the convergence behavior against the fractional order and time. We have performed our analysis in multiple subdomain cases for both in 1D \& 2D.

==> Conclusion.tex <==
\section{Conclusions}
We have extended the two classes of space-time algorithms, the Dirichlet-Neumann waveform relaxation (DNWR) and the Neumann-Neumann waveform relaxation (NNWR) algorithms, for time-fractional sub-diffusion and diffusion-wave problems. We have proved rigorously the convergence estimates for those cases in 1D, where we have taken different diffusion coefficients in different subdomains, which leads to the optimal choice of relaxation parameters for each artificial boundary. Using these optimal parameters, our estimate captures the increment of superlinear convergence rate as fractional order increases, and it goes to finite step convergence as fractional goes to two. We have numerically verified all the relaxation parameters and tested all the analytical estimates accordingly. In $2D$ case, we have taken finite lengths in $X$ axis and the entire $Y$ axis to obtain the estimates and numerically verified those.



==> Introduction.tex <==
\section{Introduction}
Parallel algorithms for fractional partial differential equations (FPDEs) \cite{xu2015parareal,lorin2020parallel,wu2017convergence} for numerical solutions are currently active research topics due to the ever-growing application of fractional PDEs in various fields like control, robotics, bio-engineering, solid and fluid mechanics, etc. \cite{hilfer2000applications,magin2004fractional,rossikhin2010application}. The numerical complexity of FPED models is much higher than its classical counterpart due to the dense matrix structure. To overcome these difficulties, parallel algorithms are a good choice to fulfill the high demand for better simulation within a reasonable time. However, due to the memory effects of fractional derivatives, it is not easy to always find an efficient parallel method, so we are forced to use classical parallel techniques for PDEs in FPDEs models whenever possible.

Two basic ways to use parallel algorithms in PDE models: one before discretization, i.e., the continuous procedure like Classical and Optimized Schwarz, Neumann-Neumann \cite{schwarz1870ueber,lions1990schwarz,bourgat1988variational}, etc. developed by Schwarz, Lions, Bourgat, and others and another one is after discretization like Additive Schwarz, Multiplicative Schwarz, Restrictive Additive Schwarz \cite{dryja1991additive,dryja1990some,cai1999restricted}, etc. introduced by Dryja, Widlund and Cai et al. And there is an ample number of other processes at both algorithmic and coding levels. Domain Decomposition (DD) algorithms on their own can handle evolution problems in discretizing time domain and are executed on each step. However, it increases the execution time and communication cost for the higher volume of transferring data among processors, so the better choice is to use waveform relaxation \cite{lelarasmee1982waveform} developed by Lelarsmee et al. and introduced in DD by Gander, Stuart, Giladi, Keller and others \cite{gander1998space,giladi2002space}. For further parallelization, one can use the parallel technique in time like Parareal, Paradiag, Paraexp, etc. introduced by Lions, Maday, Gander, and others see  \cite{lions2001resolution,maday2008parallelization,gander2013paraexp}. In this article, we have used continuous approaches, particularly Dirichlet-Neumann and Neumann-Neumann waveform relaxation, due to the efficiency of handling diffusion-type models relatively better than Classical Schwarz and Optimized Schwarz. For more details, refer to the articles \cite{gander2016dirichlet,gander2021dirichlet,mandal2017neumann}. 

Although the history of fractional calculus is quite old, dating back to $1695$ by Leibnitz, its application in electrical transmission lines was not made until $1890$ by Heaviside. The connection between fractional diffusion and anomalous diffusion under the framework of continuous time random walk was found much later by the work of Compte and Hifler \cite{hilfer1995fractional,compte1996stochastic} in 1995. Basically, random walk with the characterization of Markovian and Gaussian properties leads to the linear time dependence of the mean square displacement, i.e., $\langle x^2(t)\rangle \sim t$, which gives normal diffusion \cite{pearson1905problem,einstein1905motion,von1906kinetischen}. Moreover, when the mean square displacement is nonlinear in time, i.e., $\langle x^2(t)\rangle \sim t^{\lambda}$ (sub-diffusion: $\lambda < 1$, super-diffusion: $\lambda > 1$) then this non-Gaussian, non-Markovian, Levy Walks types model is considered as anomalous diffusion. Compte \cite{compte1996stochastic} showed that the dynamical equation of all continuous time random walk with decoupled temporal and spatial memories and with either temporal or spatial scale invariance in limiting case leads to time-fractional (Riemann-Liouville) and space fractional (Riesz) diffusion equation. In this article, we use Caputo fractional time derivative. The model we get from Compte's work using the Riemann-Liouville derivative and our model on fractional diffusion, also known as the sub-diffusion equation, using Caputo derivative are equivalent without having the forcing term for fractional time derivative order $0< \alpha < 1$, see \cite{evangelista2018fractional}. $\alpha = 1$ imply normal diffusion corresponding to $\lambda = 1$. The model with the time-fractional derivative $\alpha \in (1,2)$ is known as fractional wave, enhanced diffusion, or super-diffusion. Except $1D$, the solutions of this model in $2D$ and $3D$  do not follow the probability distribution rule, i.e., the solution may change sign, see \cite{hanygad2002multidimensional}, so in that sense $\alpha >1$ does not follow the super-diffusive random walk model corresponding to $\lambda>1$ in higher dimension. Nonetheless, this model has physical applications in viscoelasticity and constant Q seismic-wave propagation \cite{pipkin2012lectures,caputo1967linear}.

The analytic solution of the fractional diffusion wave (FDW) equation in terms of Fox's H function was first investigated by Wess and Schneider \cite{schneider1989fractional}. Mainardi \cite{mainardi1996fundamental} used Laplace transformation to obtain the fundamental solution of FDW equations in terms of the M-Wright function. Agrawal \cite{agrawal2003response} used the separation of variables technique to reduce the FDW equation in terms of the set of infinite Fractional Differential equations and then identify the eigenfunctions that produce the solutions in the form of Duhamel's integral.

From the numerical standpoint, the solution of fractional diffusion (FD) equations  Yuste and Acedo \cite{yuste2005explicit} used forward time central space with the combination of  Grunwald–Letnikov discretization of the Riemann–Liouville derivative to obtain an explicit scheme with the first order accuracy in time. Laglands and Henry \cite{langlands2005accuracy} used backward time central space with the combination of the L1 scheme developed by Oldham and Spanier for fractional time derivative to obtain a fully implicit finite difference scheme, and its unconditional stability was proved by Chen et al. \cite{chen2007fourier}. Later Stynes et al. \cite{stynes2017error}  introduced the idea of applying the graded mesh to capture the weak singularity effect in computation and showed how the order of convergence of the scheme related to the mesh grading, and they found and proved optimal mesh grading technique. Sanz-Serna \cite{sanz1988numerical} investigated the numerical solution of a partial integrodifferential equation which may be considered a $3/2$ order time fractional wave equation. Sun and Wu \cite{sun2006fully} gave a fully discrete, unconditionally stable difference scheme of order $O(t^{3-\alpha}+h^2)$ for the fractional wave equation. 

We have organized this article by introducing the model problem in Section 2. In Sections 3 \& 4, we have briefly described the DNWR and NNWR algorithms. In Section 5, we present the necessary auxiliary results for proving the main convergence theorem. In Section 6, we have considered the DNWR algorithm for two subdomain problems and prove its convergence by estimating the error. In Sections 7 \& 8, we have done the same but for the NNWR algorithm in multiple subdomains for 1D and two subdomains for 2D. In Section 9, we have chosen a particular model and verified all theoretical results with the numerical ones.


==> Numerical.tex <==
\section{Numerical Experiments}\label{Section7}
We now perform the numerical experiments to measure the convergence rate and verify the optimized relaxation parameter for DNWR and NNWR algorithms for the model problem \cite{sun2006fully}:
\begin{equation}\label{NumericalModelProblem}
\begin{cases}
  D^{2\nu}_{t}u-\nabla\cdot\left(\kappa(\boldsymbol{x})\nabla u\right) = f(\boldsymbol{x}), \qquad& (\boldsymbol{x},t)\in\Omega\times (0,T),\\
  u(\boldsymbol{x},t)=0, & (\boldsymbol{x},t) \in \partial\Omega \times (0,T), \\
  u(\boldsymbol{x},0)=g(\boldsymbol{x}), \; \partial_t u(\boldsymbol{x},0) = 0, & \boldsymbol{x}\in\Omega.
\end{cases}
\end{equation}
In the sub-diffusion case, we discretize \eqref{NumericalModelProblem} using central finite difference in space and $L1$ scheme on graded mesh, \cite{stynes2017error} for the Caputo fractional time derivative. In the diffusion-wave case, we use a fully discrete difference scheme; see \cite{sun2006fully}. We choose the spatial grid according to the subdomain sizes. When the spatial grid sizes are different for subdomains overlapping grid is used for the ghost points. Thus one can incorporate different physics of a problem on different subdomains. For more details see \cite{henshaw2009composite,giles1997stability}

\subsection{DNWR Algorithm}
We have taken the model problem ~\eqref{NumericalModelProblem} with $F(x) = \sin(\pi x/2)$ and $g(x) = 0$ on the spatial domain $\Omega = (0,2)$ and for the time window $T = 1$. The spatial grid size is $\Delta x = 0.01$, and the number of temporal grids is $2^6$ as we have chosen graded mesh, so the temporal grid size varies for the sub-diffusion case. Our experiments will illustrate the DNWR method for two subdomain cases.

In Figure~\ref{NumFig01}, we compare the convergence rate of the DNWR for different values of $\theta$ for fractional order $2\nu = 0.5$. we consider On the left, $a= 0.5, b = 1.5$, and on the middle, $a=b= 1$, and on the right $a= 1.5, b= 0.5$. We run the same set of experiments in ~\ref{NumFig02} where $2\nu = 1$ on the left and $2\nu = 1.5$ on the right, respectively, for $a<b$. The $a>b$ case behaves similarly to $a<b$. In Figure~\ref{NumFig03}, we run the same set of experiments for the heterogeneous space grid, choosing $\Delta x_1 = 0.01$ and $\Delta x_2 = 0.005$ with diffusion parameter $\kappa_{1} = 1$ and $\kappa_{2} = 0.25$. Comparing these plots, we can say that $\theta = 1/(1+\sqrt{\kappa_{1}/\kappa_{2}})$  may not always be an optimal convergence rate up to tolerance, but it gives superlinear one. For more details, see \cite{mandal2021substructuring}.

In Figure~\ref{NumFig05}, we compare the convergence rates for different values of the fractional order. We can see that the larger the fractional order, the faster the convergence. 

In Figures~\ref{NumFig06}, ~\ref{NumFig07}, ~\ref{NumFig08} and  ~\ref{NumFig09}, we compare the numerical convergence rate, theoretical convergence rate, and superlinear error bound for sub-diffusion and super-diffusion case, choosing  $\kappa_{1} = 1$ and $\kappa_{2} = 0.25$. In Figure~\ref{NumFig06} and ~\ref{NumFig07}, we show the comparison for  $a>b$, that corresponds to the case of $A = 1.5$, $B = 1$, $A > B$ in Theorem \ref{Theorem2}. We consider the initial guess $h^{(0)}(t)=1, t\in(0,T]$. 

In Figure~\ref{NumFig08} and ~\ref{NumFig09}, we repeat the experiments by swapping the roles of the two subdomains so that $a<b$. This corresponds to $A=0.5$ and $B=3$, as in Theorem~\ref{Theorem3}. The diffusion coefficients and initial guesses are the same as earlier.
\begin{figure}
  \centering
  \includegraphics[width=0.30\textwidth]{DN_alb_nu_point5_theta_vary}
  \includegraphics[width=0.30\textwidth]{DN_aeb_nu_point5_theta_vary}
  \includegraphics[width=0.30\textwidth]{DN_agb_nu_point5_theta_vary}
  \caption{Convergence of DNWR for $2\nu=0.5$ for various relaxation
    parameters $\theta$ for $T=1$, on the left for $a<b$ at the middle $a=b$ and on the right for $a>b$}
  \label{NumFig01}
\end{figure}
\begin{figure}
  \centering
  \includegraphics[width=0.45\textwidth]{DN_alb_nu_1_theta_vary}
  \includegraphics[width=0.45\textwidth]{DN_alb_nu_1point5_theta_vary}
 \caption{Convergence of DNWR for $a<b$ using various relaxation
 	parameters $\theta$ for $T=1$, on the left for $2\nu = 1$ and on the right for $2\nu = 1.5$}
  \label{NumFig02}
\end{figure}
\begin{figure}
	\centering
\includegraphics[width=0.30\textwidth]{DN_alb_nu_point5_kappa_theta_vary}
\includegraphics[width=0.30\textwidth]{DN_aeb_nu_point5_kappa_theta_vary}
\includegraphics[width=0.30\textwidth]{DN_agb_nu_point5_kappa_theta_vary}
	\caption{Convergence of DNWR for $2\nu=0.5$ using various relaxation
		parameters $\theta$ and heterogeneous space grid for $T=1$, on the left for $a<b$, middle $a=b$ and on the right for $a>b$}
	\label{NumFig03}
\end{figure}
%\begin{figure}
%	\centering
%	\includegraphics[width=0.45\textwidth]{DN_alb_kappa_same_nu_vary}
%	\includegraphics[width=0.45\textwidth]{DN_agb_kappa_same_nu_vary}
%	\caption{Convergence of DNWR for $\theta = 0.5$ using various fractional order $2\nu$ for $T=1$, on the left for $a<b$ and on the right for $a>b$}
%	\label{NumFig04}
%\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth]{DN_alb_kappa_diff_nu_vary}
	\includegraphics[width=0.45\textwidth]{DN_agb_kappa_diff_nu_vary}
	\caption{Convergence of DNWR for $\theta = 0.33$ using various fractional order $2\nu$ for $T=1$, on the left for $a<b$ and on the right for $a>b$}
	\label{NumFig05}
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=0.30\textwidth]{DN_th_vs_num_alb_nu_point2}
	\includegraphics[width=0.30\textwidth]{DN_th_vs_num_alb_nu_point5}
    \includegraphics[width=0.30\textwidth]{DN_th_vs_num_alb_nu_point8}
	\caption{Comparison for $a>b$ among numerically measured convergence rate theoretical error at $T=1$, on the left for $2\nu = 0.2$, middle for $2\nu = 0.5$ and on the right for $2\nu = 0.8$}
	\label{NumFig06}
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=0.30\textwidth]{DN_th_vs_num_alb_nu_1point2}
	\includegraphics[width=0.30\textwidth]{DN_th_vs_num_alb_nu_1point5}
	\includegraphics[width=0.30\textwidth]{DN_th_vs_num_alb_nu_1point8}
	\caption{Comparison for $a>b$ among numerically measured convergence rate theoretical error at $T=1$, on the left for $2\nu = 1.2$, middle for $2\nu = 1.5$ and on the right for $2\nu = 1.8$}
	\label{NumFig07}
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=0.30\textwidth]{DN_th_vs_num_agb_nu_point2}
	\includegraphics[width=0.30\textwidth]{DN_th_vs_num_agb_nu_point5}
	\includegraphics[width=0.30\textwidth]{DN_th_vs_num_agb_nu_point8}
	\caption{Comparison for $a<b$ among numerically measured convergence rate theoretical error at $T=1$, on the left for $2\nu = .2$, middle for $2\nu = .5$ and on the right for $2\nu = .8$}
	\label{NumFig08}
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=0.30\textwidth]{DN_th_vs_num_agb_nu_1point2}
	\includegraphics[width=0.30\textwidth]{DN_th_vs_num_agb_nu_1point5}
	\includegraphics[width=0.30\textwidth]{DN_th_vs_num_agb_nu_1point8}
	\caption{Comparison for $a<b$ among numerically measured convergence rate theoretical error at $T=1$, on the left for $2\nu = 1.2$, middle for $2\nu = 1.5$ and on the right for $2\nu = 1.8$}
	\label{NumFig09}
\end{figure}
\subsection{NNWR Algorithm in 1D}
We perform the NNWR experiment on the model problem ~\eqref{NumericalModelProblem} by choosing $F(x) = \sin(\pi x/16)$ and $g(x) = x(16-x)/64$. For the first set of experiments, the domain $\Omega = (0,16)$ is divided into five subdomains with spatial grid size according to subdomain size (mentioned below) and temporal step size $\Delta t = 0.015$ for super-diffusion on a time window $T = 4$.

In Figure~\ref{NumFig2}, we compare the error for different values of the relaxation parameter $\theta$ for equal (left) and unequal (right) subdomains with fractional order $2\nu =0.5$ with the grid size $\Delta x = 0.01$. The unequal subdomains are respectively $\Omega_1 = (0,3.5), \Omega_2 = (3.5,5.5), \Omega_3 = (5.5,10),\Omega_4 = (10,12), \Omega_5 = (12,16)$. We run the same experiments for fractional order $2\nu = 1.5$ in Figure~\ref{NumFig4}. From these experiments, we observe that $\theta = 0.25$ give the super-linear optimal convergence, and the other values of $\theta$ give linear convergence.

In Figure~\ref{NumFig5}, we compare the numerical errors for different values of the fractional order $2\nu$ for the same equal and unequal subdomains, as mentioned earlier. We observe that the large value of the fractional order gives faster convergence, which is expected as per theoretical results.

So far, we have chosen $\kappa = 1$ for NNWR experiments. Now we run the experiments by considering diffusion coefficient $\kappa$ as $\kappa_1 = 0.25, \kappa_2 = 1,\kappa_3 = 0.25,\kappa_4 = 4,\kappa_5 = 1$, and show in Figure~\ref{NumFig6}. We consider $\theta_i = 1/(2+\sqrt{\kappa_i/\kappa_{i+1}}+\sqrt{\kappa_{i+1}/\kappa_i})$ for superlinear convergence.

Finally, we compare the numerical behavior of the NNWR algorithm with the theoretical estimates obtained and plot in Figure~\ref{NumFig8} \& \ref{NumFig9}. We consider four, eight, and twelve subdomain cases. Here, we divide domain $\Omega = (0,16)$ into equal subdomain size for each case and take the diffusion coefficient $\kappa_i = 1/4^{(i-1)}, i = 1,2,...,N/2$ as shown in table~\ref{Table2}. 

\begin {table}
\begin{center}
\caption {diffusion coefficient used for different subdomains in NNWR experiments in Fig.~\ref{NumFig8} and Fig.~\ref{NumFig9}. \label{Table2}}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
No. of subdomains & $\kappa_{1}$ & $\kappa_{2}$ & $\kappa_{3}$ & $\kappa_{4}$ & $\kappa_{5}$ & $\kappa_{6}$ \tabularnewline
\hline
4 & 1,4 & 2,3 &  &  &  & \tabularnewline
\hline
8 & 1,8 & 2,7 & 3,6 & 4,5 &  &  \tabularnewline
\hline
12 & 1,12 & 2,11 & 3,10 & 4,9 & 5,8 & 6,7 \tabularnewline
\hline
\end{tabular}
\end{center}
\end {table}

\begin{figure}
  \centering
  \includegraphics[width=0.45\textwidth]{NN_kappa_equal_subdomain_equal_nu_point5_theta_vary}
  \includegraphics[width=0.45\textwidth]{NN_kappa_equal_subdomain_unequal_nu_point5_theta_vary}
  \caption{Convergence of NNWR with five subdomains for $2\nu=.5$ for $T=4$ and various
    relaxation parameters on the left equal subdomain, and on the right unequal subdomain}
  \label{NumFig2}
\end{figure}
%\begin{figure}
%	\centering
%	\includegraphics[width=0.45\textwidth]{pN_equal_nu_1}
%	\includegraphics[width=0.45\textwidth]{pN_unequal_nu_1}
%	\caption{Convergence of NNWR with four subdomains for $2\nu=1$ for $T=1$ and various
%		relaxation parameters on the left equal subdomain, and on the right unequal subdomain}
%	\label{NumFig3}
%\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth]{NN_kappa_equal_subdomain_equal_nu_1point5_theta_vary}
	\includegraphics[width=0.45\textwidth]{NN_kappa_equal_subdomain_unequal_nu_1point5_theta_vary}
	\caption{Convergence of NNWR with five subdomains for $2\nu=1.5$ for $T=4$ and various
		relaxation parameters on the left equal subdomain, and on the right unequal subdomain}
	\label{NumFig4}
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth]{NN_kappa_equal_subdomain_equal_nu_vary}
	\includegraphics[width=0.45\textwidth]{NN_kappa_equal_subdomain_unequal_nu_vary}
	\caption{Convergence of NNWR with five subdomains for $T=4$ and various
		fractional order on the left equal kappa and equal subdomain size, and on the right equal kappa and unequal subdomain size}
	\label{NumFig5}
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth]{NN_kappa_unequal_subdomain_equal_nu_vary}
	\includegraphics[width=0.45\textwidth]{NN_kappa_unequal_subdomain_unequal_nu_vary}
	\caption{Convergence of NNWR with five subdomains for $T=4$ and various
		fractional order on the left unequal kappa equal subdomain size, and on the right unequal kappa and unequal subdomain size}
	\label{NumFig6}
\end{figure}
%\begin{figure}
%	\centering
%	\includegraphics[width=0.45\textwidth]{pN_kappa_equal_nu_vary}
%	\includegraphics[width=0.45\textwidth]{pN_kappa_space_unequal_nu_vary}
%	\caption{Convergence of NNWR with four subdomains for $\theta=2.5$ for $T=1$ and various
%		fractional order on the left equal kappa and domain size, and on the right unequal kappa and domain size}
%	\label{NumFig7}
%\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=0.30\textwidth]{NN_kappa_unequal_nu_point2_subdomain_vary}
	\includegraphics[width=0.30\textwidth]{NN_kappa_unequal_nu_point5_subdomain_vary}
	\includegraphics[width=0.30\textwidth]{NN_kappa_unequal_nu_point8_subdomain_vary}
	\caption{Comparison among numerically measured convergence rate theoritical error at $T=1$, on the left for $2\nu = 0.2$, middle for $2\nu = 0.5$ and on the right for $2\nu = 0.8$}
	\label{NumFig8}
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=0.30\textwidth]{NN_kappa_unequal_nu_1point2_subdomain_vary}
	\includegraphics[width=0.30\textwidth]{NN_kappa_unequal_nu_1point5_subdomain_vary}
	\includegraphics[width=0.30\textwidth]{NN_kappa_unequal_nu_1point8_subdomain_vary}
	\caption{Comparison among numerically measured convergence rate theoritical error at $T=4$, on the left for $2\nu = 1.2$, middle for $2\nu = 1.5$ and on the right for $2\nu = 1.8$}
	\label{NumFig9}
\end{figure}

\subsection{NNWR Algorithm in 2D}
We have used the model problem ~\eqref{NumericalModelProblem} with $F(x,y) = 0$ and $g(x,y) = x(2-x)\exp(-10y^2)$ on the spatial domain $\Omega = (0,2)\times(-5,5)$ and for the time window $T = 1$. We have taken spatial grid sizes $\Delta x = 0.01$, $\Delta y = 0.1$, and the number of temporal grids is $2^8$, as we have chosen graded mesh, so temporal grid size varies for the sub-diffusion case. Our experiments will illustrate the NNWR method in 2D for two subdomains cases where $\Omega_1 = (0,0.5)\times(-5,5)$ and $\Omega_2 = (0.5,2)\times(-5,5)$. In Figure~\ref{NumFig10}, we compare the numerical error with the bounded estimate of the NNWR algorithm for different fractional order $2\nu$.  
\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth]{NN2D_kappa_equal_nu_subdiffusive}
	\includegraphics[width=0.45\textwidth]{NN2D_kappa_equal_nu_superdiffusive}
	\caption{Comparing the numerical convergence and error bound of NNWR in 2D with two subdomains for $T=1$ and various
		fractional order on the left sub-diffusive region, and on the right diffusion wave region}
	\label{NumFig10}
\end{figure}

==> Proof_NNWR.tex <==
\section{Convergence of NNWR Algorithm} \label{NNWR_con}
For the convergence study of the NNWR algorithm \eqref{NNWRD}-\eqref{NNWR2} in 1D, the domain $\Omega = (0,L)$ is subdivided into $N$ non-overlapping subdomains $\Omega_i = (x_{i-1},x_i), i = 1,2,...,N$. Define subdomain length $h_i := x_i - x_{i-1}$ and  different constant diffusion coefficients $\kappa(\boldsymbol{x},t)=\kappa_i \text{ in each } \Omega_i$. Applying the Laplace transform in time, the equations \eqref{NNWRD}-\eqref{NNWR2} reduce to:
\begin{equation}\label{NNWRL}
	\begin{array}{rcll}
		\begin{cases}
			s^{2\nu}\hat{u}_{i}^{(k)}=\kappa_i\partial_{xx}\hat{u}_{i}^{(k)}, & \textrm{in } \Omega_i,\\
			\hat{u}_{i}^{(k)} = \hat{w}_{i-1}^{(k-1)}, & \textrm{at }x_{i-1}, i \neq 1,\\
			\hat{u}_{i}^{(k)} = \hat{w}_{i}^{(k-1)}, & \textrm{at }x_{i},i\neq N,\\
		\end{cases}
	\end{array}\!\!\!\!
	\begin{array}{rcll}
		\begin{cases}
			s^{2\nu}\hat{\psi}_{i}^{(k)}=\kappa_i\partial_{xx}\hat{\psi}_{i}^{(k)}, & \textrm{in }\Omega_i,\\
			-\kappa_i\partial_{x}\hat{\psi}_{i}^{(k)} = \kappa_{i-1}\partial_{x}\hat{\psi}_{i-1}^{(k)}-\kappa_{i}\partial_{x}\hat{\psi}_{i}^{(k)}, & \textrm{at }x_{i-1},i \neq 1,\\
			\kappa_i\partial_{x}\hat{\psi}_{i}^{(k)} = \kappa_{i}\partial_{x}\hat{\psi}_{i}^{(k)}-\kappa_{i+1}\partial_{x}\hat{\psi}_{i+1}^{(k)}, & \textrm{at }x_{i},i\neq N,\\
		\end{cases}
	\end{array}
\end{equation}
except for the first and last subdomain, where the Neumann boundary condition is replaced by a homogeneous Dirichlet condition. Then the trace is updated by
\begin{equation}\label{NNWRL2}
	\hat{w}_i^{(k)}(s)= \hat{w}_i^{(k-1)}(s) - \theta_i(\hat{\psi}_{i}^{(k)}(x_i,s)+\hat{\psi}_{i+1}^{(k)}(x_i,s)),\quad i=1,\ldots,N-1.
\end{equation}
The solutions to the Dirichlet subproblems for $i=1,\ldots,N$ are respectively:
\begin{align}\label{NNWR_1}
	&\hat{u}^{(k)}_{i}(x,s)  \\
	 &=\frac{1}{\sinh(h_{i}\sqrt{\frac{s^{2\nu}}{\kappa_{i}}})}
	\left(\hat{w}^{(k-1)}_{i}(s)\sinh\left((x-x_{i-1})\sqrt{\frac{s^{2\nu}}{\kappa_{i}}}\right)
	+\hat{w}^{(k-1)}_{i-1}(s)\sinh\left((x_{i}-x)\sqrt{\frac{s^{2\nu}}{\kappa_{i}}}\right)\right) \nonumber.
\end{align}
And using the solutions \eqref{NNWR_1}, Neumann subproblems give:
\begin{align*}
	\hat{\psi}^{(k)}_{1}(x,s) &= C^{(k-1)}_{1}(s) \sinh\left((x-x_{0})\sqrt{\frac{s^{2\nu}}{\kappa_1}}\right),\\ 
	\intertext{for $i = 2,\ldots,N-1,$}
    \hat{\psi}^{(k)}_{i}(x,s) &= C^{(k-1)}_{i}(s)\cosh\left((x-x_{i-1})\sqrt{\frac{s^{2\nu}}{\kappa_{i}}}\right)+D^{(k-1)}_{i}(s)\cosh\left((x_{i}-x)\sqrt{\frac{s^{2\nu}}{\kappa_{i}}}\right), \nonumber\\
    \intertext{and}
    \hat{\psi}^{(k)}_{N}(x,s) &= D^{(k-1)}_{N}(s)\sinh\left((x_{N}-x)\sqrt{\frac{s^{2\nu}}{\kappa_N}}
    \right). \nonumber
\end{align*}
For simplification, we use the notation $\sigma_{i}:=\sinh\left(h_{i}\sqrt{s^{2\nu}/\kappa_i}\right)$ and $\gamma_{i}:=\cosh\left(h_{i}\sqrt{s^{2\nu}/\kappa_i}\right)$. Then using the boundary conditions in Neumann subproblems, we obtain:
\begin{align*}
	C^{(k-1)}_{1} & = \frac{1}{\gamma_{1}}\left(\hat{w}^{(k-1)}_{1}\left(
	\frac{\gamma_{1}}{\sigma_{1}}+\sqrt{\frac{\kappa_2}{\kappa_{1}}}\frac{\gamma_{2}}{\sigma_{2}}\right)
	-\sqrt{\frac{\kappa_2}{\kappa_{1}}}\frac{\hat{w}^{(k-1)}_{2}}{\sigma_{2}}\right),\\
	C^{(k-1)}_{i} & =  \frac{1}{\sigma_{i}}\left(\hat{w}^{(k-1)}_{i}
	\left(\frac{\gamma_{i}}{\sigma_{i}}+\sqrt{\frac{\kappa_{i+1}}{\kappa_{i}}}\frac{\gamma_{i+1}}{\sigma_{i+1}}\right)
	-\frac{\hat{w}^{(k-1)}_{i-1}}{\sigma_{i}}-\sqrt{\frac{\kappa_{i+1}}{\kappa_{i}}}\frac{\hat{w}_{i+1}}{\sigma_{i+1}}\right),\quad i = 2,\ldots,N-1, \nonumber\\
	D^{(k-1)}_{i} & =  \frac{1}{\sigma_{i}}\left(\hat{w}^{(k-1)}_{i-1}
	\left(\frac{\gamma_{i}}{\sigma_{i}}+\sqrt{\frac{\kappa_{i-1}}{\kappa_{i}}}\frac{\gamma_{i-1}}{\sigma_{i-1}}\right)
	-\sqrt{\frac{\kappa_{i-1}}{\kappa_{i}}}\frac{\hat{w}^{(k-1)}_{i-2}}{\sigma_{i-1}}-\frac{\hat{w}_{i}}{\sigma_{i}}\right),\quad i = 2,\ldots,N-1, \nonumber\\
	D^{(k-1)}_{N} & = \frac{1}{\gamma_{N}}\left(\hat{w}^{(k-1)}_{N-1}\left(
	\sqrt{\frac{\kappa_{N-1}}{\kappa_{N}}}\frac{\gamma_{N-1}}{\sigma_{N-1}}+\frac{\gamma_{N}}{\sigma_{N}}\right)
	-\sqrt{\frac{\kappa_{N-1}}{\kappa_{N}}}\frac{\hat{w}^{(k-1)}_{N-2}}{\sigma_{N-1}}\right).\nonumber
\end{align*}
Substituting $\hat{\psi}_{i}$ values in updating equation \eqref{NNWRL2} and using the identity $\gamma_{i}^{2}-\sigma_{i}^{2} = 1$, we have
\begin{align}
	\hat{w}_{1}^{(k)} &=\hat{w}_{1}^{(k-1)}-\theta_1\left(\hat{w}_{1}^{(k-1)}
	\left(2+\sqrt{\frac{\kappa_{1}}{\kappa_{2}}}\frac{\gamma_{1}\gamma_{2}}{\sigma_{1}\sigma_{2}}
	+\sqrt{\frac{\kappa_{2}}{\kappa_{1}}}\frac{\sigma_{1}\gamma_{2}}{\gamma_{1}\sigma_{2}}\right)\right. \label{NN1}\\
	&\left.\kern-\nulldelimiterspace+\frac{\hat{w}_{2}^{(k-1)}}{\sigma_{2}}\left(
	\sqrt{\frac{\kappa_{3}}{\kappa_{2}}}\frac{\gamma_{3}}{\sigma_{3}}-\sqrt{\frac{\kappa_{2}}{\kappa_{1}}}\frac{\sigma_{1}}{\gamma_{1}}\right)
	-\sqrt{\frac{\kappa_{3}}{\kappa_{2}}}\frac{\hat{w}_{3}^{(k-1)}}{\sigma_{2}\sigma_{3}}\right), \nonumber\\
		\hat{w}_{i}^{(k)}&=\hat{w}_{i}^{(k-1)}-\theta_i\left(\hat{w}_{i}^{(k-1)}
		\left(2+\left(\sqrt{\frac{\kappa_i}{\kappa_{i+1}}}+\sqrt{\frac{\kappa_{i+1}}{\kappa_{i}}}\right)\frac{\gamma_{i}\gamma_{i+1}}{\sigma_{i}\sigma_{i+1}}\right)
		+\frac{\hat{w}_{i+1}^{(k-1)}}{\sigma_{i+1}}
		\sqrt{\frac{\kappa_{i+2}}{\kappa_{i+1}}}\left(\frac{\gamma_{i+2}}{\sigma_{i+2}}-\sqrt{\frac{\kappa_{i+1}}{\kappa_{i}}}\frac{\gamma_{i}}{\sigma_{i}}\right)\right.\\
		&\left.\kern-\nulldelimiterspace+\frac{\hat{w}_{i-1}^{(k-1)}}{\sigma_{i}}
		\left(\sqrt{\frac{\kappa_{i-1}}{\kappa_{i}}}\frac{\gamma_{i-1}}{\sigma_{i-1}}-\sqrt{\frac{\kappa_{i}}{\kappa_{i+1}}}\frac{\gamma_{i+1}}{\sigma_{i+1}}\right)
		-\sqrt{\frac{\kappa_{i+2}}{\kappa_{i+1}}}\frac{\hat{w}_{i+2}^{(k-1)}}{\sigma_{i+1}\sigma_{i+2}}
		-\sqrt{\frac{\kappa_{i-1}}{\kappa_{i}}}\frac{\hat{w}_{i-2}^{(k-1)}}{\sigma_{i}\sigma_{i-1}}\right), \quad i = 2,\ldots,N-2, \nonumber\\
	\hat{w}_{N-1}^{(k)} &= \hat{w}_{N-1}^{(k-1)}-\theta_{N-1}\left(
	\hat{w}_{N-1}^{(k-1)}\left(2+\sqrt{\frac{\kappa_{N}}{\kappa_{N-1}}}\frac{\gamma_{N-1}\gamma_{N}}{\sigma_{N-1}\sigma_{N}}
	+\sqrt{\frac{\kappa_{N-1}}{\kappa_{N}}}\frac{\sigma_{N}\gamma_{N-1}}{\gamma_{N}\sigma_{N-1}}\right)\right. \label{NN3}\\
	&\left.\kern-\nulldelimiterspace+\frac{\hat{w}_{N-2}^{(k-1)}}{\sigma_{N-1}}\left(
	\sqrt{\frac{\kappa_{N-2}}{\kappa_{N-1}}}\frac{\gamma_{N-2}}{\sigma_{N-2}}-\sqrt{\frac{\kappa_{N-1}}{\kappa_{N}}}\frac{\sigma_{N}}{\gamma_{N}}\right)-\sqrt{\frac{\kappa_{N-2}}{\kappa_{N-1}}}\frac{\hat{w}_{N-3}^{(k-1)}}{\sigma_{N-1}\sigma_{N-2}}\right). \nonumber	
\end{align}
Substituting $\theta_i= \theta_i^{*} := \frac{1}{2+\sqrt{\kappa_i/\kappa_{i+1}}+\sqrt{\kappa_{i+1}/\kappa_{i}}}$ into \eqref{NN1}-\eqref{NN3} leads to the following equations:
\begin{align}
	\hat{w}_{1}^{(k)}&=-\theta_1^*\left[\hat{w}_{1}^{(k-1)}
	\left(\sqrt{\frac{\kappa_{1}}{\kappa_{2}}}\left(\frac{\gamma_{1}\gamma_{2}}{\sigma_{1}\sigma_{2}}-1\right)
	+\sqrt{\frac{\kappa_{2}}{\kappa_{1}}}\left(\frac{\sigma_{1}\gamma_{2}}{\gamma_{1}\sigma_{2}}-1\right)\right)\right. \label{NN4}\\ 
	&\left.\kern-\nulldelimiterspace+\frac{\hat{w}_{2}^{(k-1)}}{\sigma_{2}}\left(
	\sqrt{\frac{\kappa_{3}}{\kappa_{2}}}\frac{\gamma_{3}}{\sigma_{3}}-\sqrt{\frac{\kappa_{2}}{\kappa_{1}}}\frac{\sigma_{1}}{\gamma_{1}}\right)-\sqrt{\frac{\kappa_{3}}{\kappa_{2}}}\frac{\hat{w}_{3}^{(k-1)}}{\sigma_{2}\sigma_{3}}\right],\nonumber 
\end{align}
\begin{align}
	  \hat{w}_{i}^{(k)}&= -\theta_i^*\left[\hat{w}_{i}^{(k-1)}
	  \left(\sqrt{\frac{\kappa_i}{\kappa_{i+1}}}+\sqrt{\frac{\kappa_{i+1}}{\kappa_{i}}}\right)\left(\frac{\gamma_{i}\gamma_{i+1}}{\sigma_{i}\sigma_{i+1}}-1\right) +\frac{\hat{w}_{i+1}^{(k-1)}}{\sigma_{i+1}}
	  \left(\sqrt{\frac{\kappa_{i+2}}{\kappa_{i+1}}}\frac{\gamma_{i+2}}{\sigma_{i+2}}-\sqrt{\frac{\kappa_{i+1}}{\kappa_{i}}}\frac{\gamma_{i}}{\sigma_{i}}\right)\right. \\
	  &\left.\kern-\nulldelimiterspace +\frac{\hat{w}_{i-1}^{(k-1)}}{\sigma_{i}} \left(\sqrt{\frac{\kappa_{i-1}}{\kappa_{i}}}\frac{\gamma_{i-1}}{\sigma_{i-1}}-\sqrt{\frac{\kappa_{i}}{\kappa_{i+1}}}\frac{\gamma_{i+1}}{\sigma_{i+1}}\right)-\sqrt{\frac{\kappa_{i+2}}{\kappa_{i+1}}}\frac{\hat{w}_{i+2}^{(k-1)}}{\sigma_{i+1}\sigma_{i+2}}
	  -\sqrt{\frac{\kappa_{i-1}}{\kappa_{i}}}\frac{\hat{w}_{i-2}^{(k-1)}}{\sigma_{i}\sigma_{i-1}}\right],  \nonumber \\
	\hat{w}_{N-1}^{(k)}&= -\theta_{N-1}^*\left[
	\hat{w}_{N-1}^{(k-1)}\left(\sqrt{\frac{\kappa_{N}}{\kappa_{N-1}}}\left(\frac{\gamma_{N-1}\gamma_{N}}{\sigma_{N-1}\sigma_{N}}-1\right)
	+\sqrt{\frac{\kappa_{N-1}}{\kappa_{N}}}\left(\frac{\sigma_{N}\gamma_{N-1}}{\gamma_{N}\sigma_{N-1}}-1\right)\right) \right. \label{NN6}\\
	&\left.\kern-\nulldelimiterspace +\frac{\hat{w}_{N-2}^{(k-1)}}{\sigma_{N-1}}\left(
	\sqrt{\frac{\kappa_{N-2}}{\kappa_{N-1}}}\frac{\gamma_{N-2}}{\sigma_{N-2}}-\sqrt{\frac{\kappa_{N-1}}{\kappa_{N}}}\frac{\sigma_{N}}{\gamma_{N}}\right) -\sqrt{\frac{\kappa_{N-2}}{\kappa_{N-1}}}\frac{\hat{w}_{N-3}^{(k-1)}}{\sigma_{N-1}\sigma_{N-2}}\right]. \nonumber
\end{align}
With these preparation we are in position to present the following convergence theorems:
\begin{theorem}[Convergence of NNWR for subdiffusion and diffusion-wave]
	For $\theta_i = \frac{1}{2+\sqrt{\kappa_i/\kappa_{i+1}}+\sqrt{\kappa_{i+1}/\kappa_{i}}}$, the NNWR algorithm for the fractional order $ (0<\nu<1) $ in \eqref{NNWRD}-\eqref{NNWR2} converges superlinearly with the estimate:
\begin{equation}
	\max_{1 \leq i \leq N-1}\| w_i^{(k)}\|_{L^{\infty}(0,T)}\leq
	c^{k}\exp\left(-\mu (2k)^{1/(1-\nu)}\right)\max_{1 \leq i \leq N-1}\| w_i^{(0)}\|_{L^{\infty}(0,T)},
\end{equation}
where $\mu = (1-\nu)\nu^{\nu/(1-\nu)}(h_{\min}/t^{\nu})^{1/(1-\nu)}$, and value of $c$ is given in \eqref{c_val_super}.
\end{theorem}
\begin{proof}
Define $\sigma := \exp(h_{\min}s^{\nu})$ for $0<\nu<1$, where $h_{\min} = \min_{1\leq i\leq N} h_i/2/\sqrt{\kappa_i}$. Setting 
$\hat{v}^{(k)}_i(s):= \sigma^{2k}\hat{w}^{(k)}_i(s)$ reduce the equations \eqref{NN4}-\eqref{NN6} to:
\begin{align} \label{NN7}
\hat{v}^{(k)}_1(s) &= -\theta_1^{*}\left(\hat{t}_{1,1}\hat{v}^{(k-1)}_1(s)+\hat{t}_{1,2}\hat{v}^{(k-1)}_{2}(s)-\hat{t}_{1,3}\hat{v}^{(k-1)}_{3}(s)\right),  \\
\hat{v}^{(k)}_i(s) &= -\theta_i^{*}\left(\hat{t}_{i,i}\hat{v}^{(k-1)}_i(s)+\hat{t}_{i,i+1}\hat{v}^{(k-1)}_{i+1}(s)+\hat{t}_{i,i-1}\hat{v}^{(k-1)}_{i-1}(s)-\hat{t}_{i,i+2}\hat{v}^{(k-1)}_{i+2}(s)-\hat{t}_{i,i-2}\hat{v}^{(k-1)}_{i-2}(s)\right), \nonumber\\
\hat{v}^{(k)}_{N-1}(s) &= -\theta_{N-1}^{*}\left(\hat{t}_{N-1,N-1}\hat{v}^{(k-1)}_{N-1}(s)+\hat{t}_{N-1,N-2}\hat{v}^{(k-1)}_{N-2}(s)-\hat{t}_{N-1,N-3}\hat{v}^{(k-1)}_{N-3}(s)\right), \nonumber
\end{align}
where the weights are given by
\begin{gather} \label{NNWR3}
\hat{t}_{1,1} = \sigma^{2}\left(\sqrt{\frac{\kappa_1}{\kappa_{2}}}\left(\frac{\gamma_{1}\gamma_{2}}{\sigma_{1}\sigma_{2}}-1\right)+\sqrt{\frac{\kappa_2}{\kappa_{1}}}\left(\frac{\sigma_{1}\gamma_{2}}{\gamma_{1}\sigma_{2}}-1\right)\right), \,
\hat{t}_{1,2} = \frac{\sigma^{2}}{\sigma_{2}}\left(\sqrt{\frac{\kappa_3}{\kappa_{2}}}\frac{\gamma_{3}}{\sigma_{3}}-\sqrt{\frac{\kappa_2}{\kappa_{1}}}\frac{\sigma_{1}}{\gamma_{1}}\right), \\
\hat{t}_{1,3} = \frac{\sigma^{2}}{\sigma_{2}\sigma_{3}}\sqrt{\frac{\kappa_3}{\kappa_{2}}}, \nonumber 
\end{gather}
for $i = 2,\cdots,N-2$,
\begin{gather*} 
\hat{t}_{i,i} = \left(\sqrt{\frac{\kappa_i}{\kappa_{i+1}}}+\sqrt{\frac{\kappa_{i+1}}{\kappa_{i}}}\right)\sigma^{2} \left(\frac{\gamma_i \gamma_{i+1}}{\sigma_i \sigma_{i+1}}-1\right), \,
\hat{t}_{i,i+1} = \frac{\sigma^{2}}{\sigma_{i+1}}\left(\sqrt{\frac{\kappa_{i+2}}{\kappa_{i+1}}}\frac{\gamma_{i+2}}{\sigma_{i+2}}-\sqrt{\frac{\kappa_{i+1}}{\kappa_{i}}}\frac{\gamma_{i}}{\sigma_{i}}\right), \\
\hat{t}_{i,i-1} = \frac{\sigma^{2}}{\sigma_{i}}\left(\sqrt{\frac{\kappa_{i-1}}{\kappa_{i}}}\frac{\gamma_{i-1}}{\sigma_{i-1}}-\sqrt{\frac{\kappa_i}{\kappa_{i+1}}}\frac{\gamma_{i+1}}{\sigma_{i+1}}\right), \,
\hat{t}_{i,i+2} = \frac{\sigma^{2}}{\sigma_{i+1}\sigma_{i+2}}\sqrt{\frac{\kappa_{i+2}}{\kappa_{i+1}}}, \,
\hat{t}_{i,i-2} = \frac{\sigma^{2}}{\sigma_{i}\sigma_{i-1}}\sqrt{\frac{\kappa_{i-1}}{\kappa_{i}}}, \nonumber
\end{gather*}
and
\begin{gather*} 
\hat{t}_{N-1,N-1} = \sigma^{2}\left(\sqrt{\frac{\kappa_N}{\kappa_{N-1}}}\left(\frac{\gamma_{N-1}\gamma_{N}}{\sigma_{N-1}\sigma_{N}}-1\right)+\sqrt{\frac{\kappa_{N-1}}{\kappa_{N}}}\left(\frac{\sigma_{N}\gamma_{N-1}}{\gamma_{N}\sigma_{N-1}}-1\right)\right), \\
\hat{t}_{N-1,N-2} = \frac{\sigma^{2}}{\sigma_{N-1}}\left(\sqrt{\frac{\kappa_{N-2}}{\kappa_{N-1}}}\frac{\gamma_{N-2}}{\sigma_{N-2}}-\sqrt{\frac{\kappa_{N-1}}{\kappa_{N}}}\frac{\sigma_{N}}{\gamma_{N}}\right),\,
\hat{t}_{N-1,N-3} = \frac{\sigma^{2}}{\sigma_{N-1}\sigma_{N-2}}\sqrt{\frac{\kappa_{N-2}}{\kappa_{N-1}}}.
\end{gather*}
Now, we use Lemma \ref{lam_7} on \eqref{NNWR3} to obtain the following estimates:\\
for $i = 1,2,\cdots,N-1$,
\begin{align*}
	||t_{i,i}(.)||_{L^{1}(0,T)} &\leq 2\left(\sqrt{\frac{\kappa_i}{\kappa_{i+1}}}+\sqrt{\frac{\kappa_{i+1}}{\kappa_i}}\right)\left(1+\frac{D}{h_i}\right)\left(1+\frac{D}{h_{i+1}}\right)\left[e^{-2Q_i}+e^{-2Q_{i+1}}\right]=:W_{i,i}\\
\end{align*}
for $i = 1,\cdots,N-2,$
\begin{align*}
	||t_{i,i+1}(.)||_{L^{1}(0,T)} &\leq 2\left(1+\frac{D}{h_{i+1}}\right)\left[\sqrt{\frac{\kappa_{i+2}}{\kappa_{i+1}}}\left(1+\frac{D}{h_{i+2}}\right)\left(e^{-2Q_{(i+1)/2}}+e^{-2Q_{(i+1)/2,i+2}}\right)\right. \\
	&\left.\kern-\nulldelimiterspace+\sqrt{\frac{\kappa_{i+1}}{\kappa_i}}\left(1+\frac{D}{h_i}\right)\left(e^{-2Q_{(i+1)/2}}+e^{-2Q_{(i+1)/2,i}}\right)\right]=:W_{i,i+1}, \\
	||t_{i,i+2}(.)||_{L^{1}(0,T)} &\leq 4\sqrt{\frac{\kappa_{i+2}}{\kappa_{i+1}}}\left(1+\frac{D}{h_{i+1}}\right)\left(1+\frac{D}{h_{i+2}}\right)\left(e^{-(Q_{i+1}+Q_{i+2})}\right)=:W_{i,i+2},
\end{align*}
for $i = 2,\cdots,N-1,$
\begin{align*}
	||t_{i,i-1}(.)||_{L^{1}(0,T)} &\leq 2\left(1+\frac{D}{h_{i}}\right)\left[\sqrt{\frac{\kappa_{i-1}}{\kappa_{i}}}\left(1+\frac{D}{h_{i-1}}\right)\left(e^{-2Q_{i/2}}+e^{-2Q_{i/2,i-1}}\right)\right. \\
	&\left.\kern-\nulldelimiterspace+\sqrt{\frac{\kappa_{i}}{\kappa_{i+1}}}\left(1+\frac{D}{h_{i+1}}\right)\left(e^{-2Q_{i/2}}+e^{-2Q_{i/2,i+1}}\right)\right]=:W_{i,i-1}, \\
	||t_{i,i-2}(.)||_{L^{1}(0,T)} &\leq 4\sqrt{\frac{\kappa_{i-1}}{\kappa_{i}}}\left(1+\frac{D}{h_{i-1}}\right)\left(1+\frac{D}{h_{i}}\right)\left(e^{-(Q_{i-1}+Q_{i})}\right)=:W_{i,i-2},
\end{align*}
where $D = \frac{T^{\nu}\Gamma(2-\nu)}{2\mu^{(1-\nu)}}$, and we use the following notation for convenience: $Q_j =\mu \left[\frac{h_j-h}{t^{\nu}}\right]^{1/(1-\nu)}$, $Q_{j/2} = \mu\left[\frac{h_j/2 - h}{t^{\nu}}\right]^{1/(1-\nu)},$ $ Q_{j/2,k} = \mu\left[\frac{h_j/2 + h_k - h}{t^{\nu}}\right]^{1/(1-\nu)}$.
After taking the inverse Laplace transform in equations \eqref{NN7} and using the part (iii) of Lemma \ref{SimpleLaplaceLemma} we have:
\begin{align} \label{NNWR4}
	||v_1^{(k)}(.)||_{L^{\infty}(0,T)} &\leq c_1 \max_{1 \leq j \leq N-1}||v_1^{(k-1)}(.)||_{L^{\infty}(0,T)}, \nonumber\\
	||v_i^{(k)}(.)||_{L^{\infty}(0,T)} &\leq c_i \max_{1 \leq j \leq N-1}||v_j^{(k-1)}(.)||_{L^{\infty}(0,T)},  \\
	||v_{N-1}^{(k)}(.)||_{L^{\infty}(0,T)} &\leq c_{N-1} \max_{1 \leq j \leq N-1}||v_j^{(k-1)}(.)||_{L^{\infty}(0,T)}. \nonumber
\end{align}
 where
\begin{align*}
	c_1 &=  W_{1,1} + W_{1,1+1} + W_{1,1+2}, \\
	c_i &= W_{i,i} + W_{i,i-1} + W_{i,i+1} + W_{i,i-2} + W_{i,i+2}, \quad i = 2,\cdots,N-2,\\
	c_{N-1} &= W_{N-1,N-1} + W_{N-1,N-2} + W_{N-1,N-3}. \\
\end{align*}
Define for $i = 2,\cdots,N-2$
\begin{equation} \label{c_val_super}
	c := \max\{\theta^*_1c_1,\theta^*_ic_i,\theta^*_{N-1}c_{N-1}\}.
\end{equation}
Then from equations \eqref{NNWR4}, we have 
\[||v_i^{(k)}(.)||_{L^{\infty}(0,T)} \leq c \max_{1 \leq j \leq N-1}||v_j^{(k-1)}(.)||_{L^{\infty}(0,T)}\]
which further yields
\begin{equation*}
	\max_{1 \leq i \leq N-1}||v_i^{(k)}(.)||_{L^{\infty}(0,T)} \leq c^k \max_{1 \leq j \leq N-1}||v_j^{(0)}(.)||_{L^{\infty}(0,T)}.
\end{equation*}
Now since
\[ w_i^{(k)}(t) = \left(\phi^{2k}*v_i^{(k)}\right)(t) = \int_0^{\infty}\phi^{2k}(t-\tau)v_i^k(\tau)d\tau,\]
with $\phi^{k} = \mathcal{L}^{-1}\left\{\exp(-kh_{\min}s^{\nu})\right\}$ for $0<\nu <1.$
And finally using part (iii) of Lemma \ref{SimpleLaplaceLemma} and part (iii) of Lemma \ref{invL_exp} we have the proof.	
\hfill\end{proof}



==> Proof_NNWR2D.tex <==
\section{Convergence of NNWR Algorithm in 2D} \label{NNWR2D_con}
For the convergence study of the NNWR \eqref{NNWRD}-\eqref{NNWR2} algorithm in two subdomains in 2D domain $\Omega = (-a,b)\times \mathbb{R}$ is divided into two non-overlapping subdomains $\Omega_1 = (-a,0)\times \mathbb{R} \textrm{ and } \Omega_2 = (0,b)\times \mathbb{R}$. For convenience, we take $\kappa(\boldsymbol{x},t)=\kappa \text{ in } \Omega$. Let, $u_1,\psi_1$ are restricted to $\Omega_{1}$ and $u_2,\psi_2$ are restricted to $\Omega_{2}$. We apply Fourier transform in $y$ and then Laplace transform in $t$ to reduce the iteration as follows:
\begin{equation}\label{NNWR2DL}
	\begin{array}{rcll}
		\begin{cases}
			(s^{2\nu}+\kappa\xi^2)\widehat{\mathcal{F}\{u_1\}}^{(k)} = \kappa\partial_{xx}\widehat{\mathcal{F}\{u_1\}}^{(k)},\\
			\widehat{\mathcal{F}\{u_1\}}^{(k)}(-a,s,\xi) = 0,\\
			\widehat{\mathcal{F}\{u_1\}}^{(k)}(0,s,\xi) = \widehat{\mathcal{F}\{w\}}^{(k-1)}(s,\xi),
		\end{cases}
	\end{array}\!\!
	\begin{array}{rcll}
		\begin{cases}
			(s^{2\nu}+\kappa\xi^2)\widehat{\mathcal{F}\{u_2\}}^{(k)} = \kappa\partial_{xx}\widehat{\mathcal{F}\{u_2\}}^{(k)},\\
			\widehat{\mathcal{F}\{u_2\}}^{(k)}(0,s,\xi) = \widehat{\mathcal{F}\{w\}}^{(k-1)}(s,\xi),\\
			\widehat{\mathcal{F}\{u_2\}}^{(k)}(b,s,\xi) = 0,
		\end{cases}
	\end{array}
\end{equation}
\begin{equation}\label{NNWR2DR}
	\begin{array}{rcll}
		\begin{cases}
			(s^{2\nu}+\kappa\xi^2)\widehat{\mathcal{F}\{\psi_1\}}^{(k)} = \kappa\partial_{xx}\widehat{\mathcal{F}\{\psi_1\}}^{(k)},\\
			\widehat{\mathcal{F}\{\psi_1\}}^{(k)}(-a,s,\xi) = 0,\\
			\partial_{x}\widehat{\mathcal{F}\{\psi_1\}}^{(k)} =
			\partial_{x}\widehat{\mathcal{F}\{u_1\}}^{(k)}-\partial_{x}\widehat{\mathcal{F}\{u_2\}}^{(k)},
		\end{cases}
	\end{array}\!\!\!\!\!\!\!\!\!
	\begin{array}{rcll}
		\begin{cases}
			(s^{2\nu}+\kappa\xi^2)\widehat{\mathcal{F}\{\psi_2\}}^{(k)} = \kappa\partial_{xx}\widehat{\mathcal{F}\{\psi_2\}}^{(k)},\\
			\partial_{x}\widehat{\mathcal{F}\{\psi_2\}}^{(k)} =
			\partial_{x}\widehat{\mathcal{F}\{u_2\}}^{(k)}-\partial_{x}\widehat{\mathcal{F}\{u_1\}}^{(k)},\\
			\widehat{\mathcal{F}\{\psi_2\}}^{(k)}(b,s,\xi) = 0,
		\end{cases}
	\end{array}
\end{equation}
followed by the updating step:
\begin{equation}\label{NNWR2DL2}
	\widehat{\mathcal{F}\{w\}}^{(k)}(s,\xi)= \widehat{\mathcal{F}\{w\}}^{(k-1)}(s,\xi) - \theta\left(\widehat{\mathcal{F}\{\psi_1\}}^{(k)}(0,\xi,s)+\widehat{\mathcal{F}\{\psi_2\}}^{(k)}(0,\xi,s)\right).
\end{equation}
After finding the solutions of \eqref{NNWR2DL}\&\eqref{NNWR2DR} and substituting in \eqref{NNWR2DL2}, we obtain
\begin{equation*}
	\widehat{\mathcal{F}\{w\}}^{(k)} = \left[1-\theta\left(2+\frac{\tanh(B\sqrt{s^{2\nu}+\kappa\xi^2})}{\tanh(A\sqrt{s^{2\nu}+\kappa\xi^2})}+\frac{\tanh(A\sqrt{s^{2\nu}+\kappa\xi^2})}{\tanh(B\sqrt{s^{2\nu}+\kappa\xi^2})}\right)\right]\widehat{\mathcal{F}\{w\}}^{(k-1)},
\end{equation*}
where, $A:=a/\sqrt{\kappa}$ and $B:=b/\sqrt{\kappa}$. Then put $\theta = 1/4$, we obtain
\begin{equation*}
	\widehat{\mathcal{F}\{w\}}^{(k)} = \frac{\sinh^2((A-B)\sqrt{s^{2\nu}+\kappa\xi^2})}{\sinh(2A\sqrt{s^{2\nu}+\kappa\xi^2})\sinh(2B\sqrt{s^{2\nu}+\kappa\xi^2})}\widehat{\mathcal{F}\{w\}}^{(k-1)},
\end{equation*}
that further leads to the relation
\begin{equation}\label{NNWR_2d_1}
	\widehat{\mathcal{F}\{w\}}^{(k)} = \frac{\sinh^{2k}((A-B)\sqrt{s^{2\nu}+\kappa\xi^2})}{\sinh^k(2A\sqrt{s^{2\nu}+\kappa\xi^2})\sinh^k(2B\sqrt{s^{2\nu}+\kappa\xi^2})}\widehat{\mathcal{F}\{w\}}^{(0)}.
\end{equation}
 We have the followings convergence theorems:
 \begin{theorem}[Convergence of NNWR in 2D]
 	For $\theta = 1/4$, the NNWR algorithm in 2D for sub-diffusion problem converges superlinearly with the estimate:
 	\begin{equation*}
 		\|w^{(k)}\| \leq \left[\frac{\left(1+\exp\left(-P(2|B-A|)^{1/(1-\nu)}\right)\right)^2}{\left(1-\exp(-PEF)\right)\left(1-\exp(-PEH)\right)}\right]^k \exp(-2PEk^{1/(1-\nu)})\|w^{(0)}\|,
 	\end{equation*}
where, $E = (2\min(A,B))^{1/(1-\nu)}$, $F = \left[(2\max(A,B)/\min(A,B) + k)^c - k^c\right]^{1/c(1-\nu)}$, $H = \left[(2 + k)^c - k^c\right]^{1/c(1-\nu)}$, $c = \floor*{\frac{1}{1-\nu}}$, and $P = (1-\nu)(\nu/t)^{\nu/(1-\nu)}$.
A similar estimate holds for diffusion wave case for all $k >K$ s.t. $kB >\nu^{1-\nu}t^{\nu}/(1-\nu)^{1-\nu}\nu^{\nu}$. 
 \end{theorem}
\begin{proof}
	When $A>B$, we choose  $\widehat{\mathcal{F}\{v\}}^{(k)} := \sinh^k(2B\sqrt{s^{2\nu}+\kappa\xi^2})\widehat{\mathcal{F}\{w\}}^{(k)}$; therefore, equation \eqref{NNWR_2d_1} reduce to:
	\begin{align} \label{2DNN3}
		&\widehat{\mathcal{F}\{v\}}^{(k)}  \\ 
		&=\frac{\sinh^{2k}((A-B)\sqrt{s^{2\nu}+\kappa\xi^2})}{\sinh^k(2A\sqrt{s^{2\nu}+\kappa\xi^2})}\widehat{\mathcal{F}\{v\}}^{(0)}  \nonumber\\
		&= \frac{1}{2^k}\sum_{i=0}^{2k}(-1)^i \binom{2k}{i}\sum_{m=0}^{\infty}\binom{m+k-1}{m}\mathcal{L}^{-1}\{\exp(-2(2mA+kB+i(A-B))\sqrt{s^{2\nu}+\kappa\xi^2})\}\widehat{\mathcal{F}\{v\}}^{(0)}.\nonumber
	\end{align}
%Now, taking the inverse Laplace transform and using the part (i) of Lemma \ref{invL_sinh_sinh}, we have
% 	\begin{align*}
% 		&\mathcal{F}\{v\}^{(k)} \\
% 		&= \frac{1}{2^k}\sum_{i=0}^{2k}(-1)^i \binom{2k}{i}\sum_{m=0}^{\infty}\binom{m+k-1}{m}\mathcal{L}^{-1}\{\exp(-2(2mA+kB+i(A-B))\sqrt{s^{2\nu}+\kappa\xi^2})\}\ast\mathcal{F}\{v\}^{(0)}
% 	\end{align*}
% $\exists k > K $ when we do the inverse Fourier transform we have:
% \begin{equation*}
% 	|v^{(k)}| \leq \frac{1}{2^k}\sum_{i=0}^{2k} \binom{2k}{i}\sum_{m=0}^{\infty}\binom{m+k-1}{m}\|\mathcal{L}^{-1}\{\exp(-2(2mA+kB+i(A-B))s^{\nu})\}\|\|v^{(0)}\|
% \end{equation*}
When $0< \nu \leq 1/2$, using the part (i) of Lemma \ref{estimate_9} and $P = (1-\nu)(\nu/t)^{1/(1-\nu)}$ on equation \eqref{2DNN3} gives
 \begin{align} \label{2DNN1}
	&|v^{(k)}| \\
    &\leq \frac{1}{2^k}\sum_{i=0}^{2k} \binom{2k}{i}\sum_{m=0}^{\infty}\binom{m+k-1}{m}\exp(-P(2(2mA+kB+i(A-B)))^{1/(1-\nu)})\|v^{(0)}\| \nonumber\\
	& \leq \frac{1}{2^k}\sum_{i=0}^{2k}\exp(-P(2(i(A-B)))^{1/(1-\nu)})\sum_{m=0}^{\infty}\binom{m+k-1}{m}\exp(-P(2(2mA+kB))^{1/(1-\nu)})\|v^{(0)}\|. \nonumber
\end{align}
Using \eqref{lam_4_2} we obtain:
\begin{align*}
	|v^{(k)}| \leq \frac{1}{2^k}\left[1+\exp\left(-P(2(A-B))^{1/(1-\nu)}\right)\right]^{2k}\frac{\exp(-PE_1k^{1/(1-\nu)})}{\left(1-\exp(-PE_1F_1)\right)^k}\|v^{(0)}\|, \nonumber
\end{align*}
where, $E_1 = (2B)^{1/(1-\nu)}$ and $F_1 = \left[(2A/B + k)^c - k^c\right]^{1/c(1-\nu)}$.\\
When $1/2< \nu \leq 1$, using the part (ii) of Lemma \ref{estimate_9} and $P = (1-\nu)(\nu/t)^{1/(1-\nu)}$ and $\exists k > K $ s.t. for $kB >\nu^{1-\nu}t^{\nu}/(1-\nu)^{1-\nu}\nu^{\nu}$ similar result as \eqref{2DNN1} holds for \eqref{2DNN3}.
Now $\hat{\tilde{w}}^{(k)} = \frac{1}{\sinh^k(2B\sqrt{s^{2\nu}+\kappa\xi^2})}\hat{\tilde{v}}^{(k)}$.
Using the similar estimate, we obtain
\begin{equation} \label{2DNN2}
	|w^{(k)}| \leq \left[\frac{2}{1-\exp(-PE_1H)}\right]^k \exp(-PEk^{1/(1-\nu)})\|v^{(k)}\|,
\end{equation}
where, $H = \left[(2 + k)^c - k^c\right]^{1/c(1-\nu)}$.
Finally, combining \eqref{2DNN1} and \eqref{2DNN2} and taking the norm on left hand side we get:
\begin{equation} \label{2DNN4}
	\|w^{(k)}\| \leq \left[\frac{\left(1+\exp\left(-P(2(A-B))^{1/(1-\nu)}\right)\right)^2}{\left(1-\exp(-PE_1F_1)\right)\left(1-\exp(-PE_1H)\right)}\right]^k \exp(-2PE_1k^{1/(1-\nu)})\|w^{(0)}\|.
\end{equation}
Similarly, for $B>A$ we can prove
\begin{equation}\label{2DNN5}
	\|w^{(k)}\| \leq \left[\frac{\left(1+\exp\left(-P(2(B-A))^{1/(1-\nu)}\right)\right)^2}{\left(1-\exp(-PE_2F_2)\right)\left(1-\exp(-PE_2H)\right)}\right]^k \exp(-2PE_2k^{1/(1-\nu)})\|w^{(0)}\|,
\end{equation}
where, $E_2 = (2A)^{1/(1-\nu)}$ and $F_2 = \left[(2B/A + k)^c - k^c\right]^{1/c(1-\nu)}$.
Finally, combining \eqref{2DNN4} \& \eqref{2DNN5} we have the proof for all $k \in \mathbb{N}$ for subdiffusion case and for all $k >K$ s.t. $kB >\nu^{1-\nu}t^{\nu}/(1-\nu)^{1-\nu}\nu^{\nu}$ for diffusion wave case.
\hfill\end{proof}	



%\begin{theorem}[Convergence of NNWR for sub-diffusion]
%	Interface error after $k$th iteration $\left\{w_i^{(k)}\right\}_{i=1}^{N-1}$ for the error equation in sub-diffusion $ (0<\nu\leq1/2) $ case of the NNWR algorithm \eqref{NNWRD}-\eqref{NNWR2} with the initial guess $\left\{w_i^{(0)}\right\}_{i=1}^{N-1}$ along the interface $\left\{x_i\right\}_{i=1}^{N-1}$ satisfy the super-linear bound:
%	\begin{equation}
%		\| w^{(k)}\|_{L^{\infty}(0,T;L^2(-\infty,\infty))}\leq
%		c^{k}\exp\left(-\alpha k^{1/(1-\nu)}\right)\| w^{(0)}\|_{L^{\infty}(0,T;L^2(-\infty,\infty))},
%	\end{equation}
%	where, $\alpha = (1-\nu)\nu^{\nu/(1-\nu)}(h_{\min}/t^{\nu})^{1/(1-\nu)}$ and value of $c$ is given in \eqref{c_val_super}.
%\end{theorem}
%\begin{proof}
%	Define $\sigma := \exp(h_{\min}\sqrt{s^{2\nu} + \kappa\xi^2})$ for $0<\nu<1$ where $h_{\min} = min_{1\leq i\leq N} h_i/\sqrt{\kappa}$, setting 
%	$\hat{\tilde{v}}^{(k)}_i(\xi,s):= \sigma^{2k}\hat{\tilde{w}}^{(k)}_i(\xi,s)$ and performing the same procedure leads to find the following estimates named as $W_{i,j}$:
%	\begin{align}
%		\hat{\tilde{v}}^{(k)}_1 &= -\theta^{*}\left(\hat{\tilde{t}}_{1,1}\hat{\tilde{v}}^{(k-1)}_1+\hat{\tilde{t}}_{1,2}\hat{\tilde{v}}^{(k-1)}_{2}-\hat{\tilde{t}}_{1,3}\hat{\tilde{v}}^{(k-1)}_{3}\right), \label{NN2D7} \\
%		\hat{\tilde{v}}^{(k)}_i &= -\theta^{*}\left(\hat{\tilde{t}}_{i,i}\hat{\tilde{v}}^{(k-1)}_i+\hat{\tilde{t}}_{i,i+1}\hat{v}^{(k-1)}_{i+1}+\hat{\tilde{t}}_{i,i-1}\hat{\tilde{v}}^{(k-1)}_{i-1}-\hat{\tilde{t}}_{i,i+2}\hat{\tilde{v}}^{(k-1)}_{i+2}-\hat{\tilde{t}}_{i,i-2}\hat{\tilde{v}}^{(k-1)}_{i-2}\right), \nonumber\\
%		\hat{\tilde{v}}^{(k)}_{N-1} &= -\theta^{*}\left(\hat{\tilde{t}}_{N-1,N-1}\hat{\tilde{v}}^{(k-1)}_{N-1}+\hat{\tilde{t}}_{N-1,N-2}\hat{\tilde{v}}^{(k-1)}_{N-2}-\hat{\tilde{t}}_{N-1,N-3}\hat{\tilde{v}}^{(k-1)}_{N-3}\right), \nonumber
%	\end{align}
%	where we define
%	\begin{gather}
%		\hat{\tilde{t}}_{1,1} = \sigma^{2}\left(\left(\frac{\gamma_{1}\gamma_{2}}{\sigma_{1}\sigma_{2}}-1\right)+\left(\frac{\sigma_{1}\gamma_{2}}{\gamma_{1}\sigma_{2}}-1\right)\right), \,
%		\hat{t}_{1,2} = \frac{\sigma^{2}}{\sigma_{2}}\left(\frac{\gamma_{3}}{\sigma_{3}}-\frac{\sigma_{1}}{\gamma_{1}}\right), \\
%		\hat{t}_{1,3} = \frac{\sigma^{2}}{\sigma_{2}\sigma_{3}}, \nonumber 
%	\end{gather}
%	for $i = 1,\cdots,N-2$,
%	\begin{gather*} 
%		\hat{t}_{i,i} = 2\sigma^{2} \left(\frac{\gamma_i \gamma_{i+1}}{\sigma_i \sigma_{i+1}}-1\right), \,
%		\hat{t}_{i,i+1} = \frac{\sigma^{2}}{\sigma_{i+1}}\left(\frac{\gamma_{i+2}}{\sigma_{i+2}}-\frac{\gamma_{i}}{\sigma_{i}}\right), \\
%		\hat{t}_{i,i-1} = \frac{\sigma^{2}}{\sigma_{i}}\left(\frac{\gamma_{i-1}}{\sigma_{i-1}}-\frac{\gamma_{i+1}}{\sigma_{i+1}}\right), \,
%		\hat{t}_{i,i+2} = \frac{\sigma^{2}}{\sigma_{i+1}\sigma_{i+2}}, \,
%		\hat{t}_{i,i-2} = \frac{\sigma^{2}}{\sigma_{i}\sigma_{i-1}}, \nonumber
%	\end{gather*}
%	and
%	\begin{gather*} 
%		\hat{t}_{N-1,N-1} = \sigma^{2}\left(\left(\frac{\gamma_{N-1}\gamma_{N}}{\sigma_{N-1}\sigma_{N}}-1\right)+\left(\frac{\sigma_{N}\gamma_{N-1}}{\gamma_{N}\sigma_{N-1}}-1\right)\right), \\
%		\hat{t}_{N-1,N-2} = \frac{\sigma^{2}}{\sigma_{N-1}}\left(\frac{\gamma_{N-2}}{\sigma_{N-2}}-\frac{\sigma_{N}}{\gamma_{N}}\right),\,
%		\hat{t}_{N-1,N-3} = \frac{\sigma^{2}}{\sigma_{N-1}\sigma_{N-2}}.
%	\end{gather*}
%	Now  
%	\begin{align*}
%		&\hat{\tilde{t}}_{1,1}\\ &= \sigma^{2}\left(\left(\frac{\gamma_{1}\gamma_{2}}{\sigma_{1}\sigma_{2}}-1\right)+\left(\frac{\sigma_{1}\gamma_{2}}{\gamma_{1}\sigma_{2}}-1\right)\right),\\
%		&= \frac{2(\exp(-2(h_1-h)\sqrt{s^{2\nu}+\kappa\xi^2})+\exp(-2(h_2-h)\sqrt{s^{2\nu}+\kappa\xi^2}))}{(1-\exp(-2h_1\sqrt{s^{2\nu}+\kappa\xi^2}))(1-\exp(-2h_2\sqrt{s^{2\nu}+\kappa\xi^2}))}\\
%		&+\frac{2(\exp(-2(h_2-h)\sqrt{s^{2\nu}+\kappa\xi^2})-\exp(-2(h_1-h)\sqrt{s^{2\nu}+\kappa\xi^2}))}{(1+\exp(-2h_1\sqrt{s^{2\nu}+\kappa\xi^2}))(1-\exp(-2h_2\sqrt{s^{2\nu}+\kappa\xi^2}))}.
%	\end{align*}
%	now, $\hat{\tilde{t}}_{1,1}\hat{\tilde{v}}_{1}$ can be written as $(A_1+A_2+A_3+A_4)\hat{\tilde{v}}_{1}$. Where :
%	\begin{align*}
%		A_1 &= \frac{2\exp(-2(h_1-h)\sqrt{s^{2\nu}+\kappa\xi^2})}{(1-\exp(-2h_1\sqrt{s^{2\nu}+\kappa\xi^2}))(1-\exp(-2h_2\sqrt{s^{2\nu}+\kappa\xi^2}))},\\
%		A_2 &= \frac{2\exp(-2(h_2-h)\sqrt{s^{2\nu}+\kappa\xi^2})}{(1-\exp(-2h_1\sqrt{s^{2\nu}+\kappa\xi^2}))(1-\exp(-2h_2\sqrt{s^{2\nu}+\kappa\xi^2}))}, \\
%		A_3 &=  \frac{2\exp(-2(h_2-h)\sqrt{s^{2\nu}+\kappa\xi^2})}{(1+\exp(-2h_1\sqrt{s^{2\nu}+\kappa\xi^2}))(1-\exp(-2h_2\sqrt{s^{2\nu}+\kappa\xi^2}))},\\
%		A_4 &= \frac{-2\exp(-2(h_1-h)\sqrt{s^{2\nu}+\kappa\xi^2})}{(1+\exp(-2h_1\sqrt{s^{2\nu}+\kappa\xi^2}))(1-\exp(-2h_2\sqrt{s^{2\nu}+\kappa\xi^2}))}.
%	\end{align*}
%	Now $A_1\hat{\tilde{v}}_{1}$ can be written as $A_{11}A_{12}\hat{\tilde{v}}_{1}$. Now, using the Lemma \ref{estimate10} we can write:
%	$\|A_1v_{1}\| \leq \|A_{11}\|\|A_{12}v_{1}\| \leq \|A_{11}\|\|A_{12}\|\|v_{1}\| $.
%	Now, repeatedly using Lemma \ref{estimate10} we have the following result:
%	\begin{align*}
%		||v_1^{(k)}(.,.)|| &\leq W_{1,1}||v_1^{(k-1)}(.,.)|| + W_{1,2}||v_2^{(k-1)}(.,.)||+W_{1,3}||v_3^{(k-1)}(.,.)||, \\
%		||v_i^{(k)}(.,.)|| &\leq W_{i,i}||v_i^{(k-1)}(.,.)|| + W_{i,i+1}||v_{i+1}^{(k-1)}(.,.)||+W_{i,i-1}||v_{i-1}^{(k-1)}(.,.)||\\
%		&+ W_{i,i+2}||v_{i+2}^{(k-1)}(.,.)||+W_{i,i-2}||v_{i-2}^{(k-1)}(.,.)||, \\
%		||v_{N-1}^{(k)}(.,.)|| &\leq W_{N-1,N-1}||v_{N-1}^{(k-1)}(.,.)|| + W_{N-1,N-2}||v_{N-2}^{(k-1)}(.,.)||+W_{N-1,N-3}||v_{N-3}^{(k-1)}(.,.)||.
%	\end{align*}
%	where $W_{i,j}$ for sub-diffusion case are defined by:
%	\begin{align*}
%		W_{i,i} &:=  4\left(1+\frac{D}{h_i}\right)\left(1+\frac{D}{h_{i+1}}\right)\left[\exp(-2M(h_i-h)^{\beta})+\exp(-2M(h_{i+1}-h)^{\beta})\right]\\
%		%&\left.\kern-\nulldelimiterspace\left[\exp\left(-2\left(\frac{\beta(h_i-h)}{t^{\nu}}\right)\right)\right] \\
%		W_{i,i+1} &:= 4\left(1+\frac{D}{h_{i}}\right)\left(1+\frac{D}{h_{i+1}}\right)\left(1+\frac{D}{h_{i+2}}\right)\left[\exp\left(-3M\left(\frac{h_{i+1}+2h_{i+2}-2h}{3}\right)^{\beta}\right)\right.\\
%		&\left.\kern-\nulldelimiterspace+\exp\left(-3M\left(\frac{h_{i+1}+2h_{i+2}-2h}{3}\right)^{\beta}\right)\right]. \\
%		W_{i,i-1} &:= 4\left(1+\frac{D}{h_{i-1}}\right)\left(1+\frac{D}{h_{i}}\right)\left(1+\frac{D}{h_{i+1}}\right)\left[\exp\left(-3M\left(\frac{h_{i}+2h_{i+1}-2h}{3}\right)^{\beta}\right)\right.\\
%		&\left.\kern-\nulldelimiterspace+\exp\left(-3M\left(\frac{h_{i}+2h_{i-1}-2h}{3}\right)^{\beta}\right)\right]. \\
%		W_{i,i+2} &:= 2\left(1+\frac{D}{h_{i+1}}\right)\left(1+\frac{D}{h_{i+2}}\right)\exp\left(-2M\left(\frac{h_{i+1}+h_{i+2}-2h}{2}\right)^{\beta}\right), \\
%		W_{i,i-2} &:= 2\left(1+\frac{D}{h_{i-1}}\right)\left(1+\frac{D}{h_{i}}\right)\exp\left(-2M\left(\frac{h_{i-1}+h_{i}-2h}{2}\right)^{\beta}\right),
%	\end{align*}
%	and for super-diffusion case $W_{i,j}$ are defined by:
%	\begin{align*}
%		W_{i,i} &:=  8\left(1+Ct+\frac{D}{h_i}\right)\left(1+Ct+\frac{D}{h_{i+1}}\right)\\
%		%&\left.\kern-\nulldelimiterspace\left[\exp\left(-2\left(\frac{\beta(h_i-h)}{t^{\nu}}\right)\right)\right] \\
%		W_{i,i+1} &:= 8\left(1+Ct+\frac{D}{h_{i}}\right)\left(1+Ct+\frac{D}{h_{i+1}}\right)\left(1+Ct+\frac{D}{h_{i+2}}\right).\\
%		W_{i,i-1} &:= 8\left(1+Ct+\frac{D}{h_{i-1}}\right)\left(1+Ct+\frac{D}{h_{i}}\right)\left(1+Ct+\frac{D}{h_{i+1}}\right),\\
%		W_{i,i+2} &:= 2\left(1+Ct+\frac{D}{h_{i+1}}\right)\left(1+Ct+\frac{D}{h_{i+2}}\right), \\
%		W_{i,i-2} &:= 2\left(1+Ct+\frac{D}{h_{i-1}}\right)\left(1+Ct+\frac{D}{h_{i}}\right),
%	\end{align*}
%	where $\beta = 1/(1-\nu),D = \frac{T^{\nu}\Gamma(2-\nu)}{2\beta}$ and $p = (\nu)^{\nu}(1-\nu)^{(1-\nu)}$ and we use the following notation for convenience, $M_j = \left[\frac{p}{t^{\nu}}\right]^{1/(1-\nu)}$.
%	Thus we have
%	\begin{align*}
%		||v_1^{(k)}(.)||_{L^{\infty}(0,T)} &\leq c_1 \max_{1 \leq j \leq N-1}||v_1^{(k-1)}(.)||_{L^{\infty}(0,T)}, \\
%		||v_i^{(k)}(.)||_{L^{\infty}(0,T)} &\leq c_i \max_{1 \leq j \leq N-1}||v_j^{(k-1)}(.)||_{L^{\infty}(0,T)}, \\
%		||v_{N-1}^{(k)}(.)||_{L^{\infty}(0,T)} &\leq c_{N-1} \max_{1 \leq j \leq N-1}||v_j^{(k-1)}(.)||_{L^{\infty}(0,T)}.
%	\end{align*}
%	where,
%	\begin{align*}
%		c_1 &=  W_{1,1} + W_{1,1+1} + W_{1,1+2}, \\
%		c_i &= W_{i,i} + W_{i,i-1} + W_{i,i+1} + W_{i,i-2} + W_{i,i+2}, \quad i = 2,\cdots,N-2,\\
%		c_{N-1} &= W_{N-1,N-1} + W_{N-1,N-2} + W_{N-1,N-3}. \\
%	\end{align*}
%	Define 
%	\begin{equation} \label{c_val_super2D}
%		c := \max\{\theta^*_1c_1,\theta^*_ic_i,\theta^*_{N-1}c_{N-1}\}.
%	\end{equation}
%	Then we have 
%	\[||v_i^{(k)}(.)||_{L^{\infty}(0,T;L^{\infty})} \leq c \max_{1 \leq j \leq N-1}||v_j^{(k-1)}(.)||_{L^{\infty}(0,T;L^{\infty})}\]
%	by substitution we obtain 
%	\begin{equation*}
%		\max_{1 \leq i \leq N-1}||v_i^{(k)}(.)||_{L^{\infty}(0,T;L^{\infty})} \leq c^k \max_{1 \leq j \leq N-1}||v_j^{(0)}(.)||_{L^{\infty}(0,T;L^{\infty})}.
%	\end{equation*}
%	Now since
%	\[ \tilde{w}_i^{(k)}(t,\xi) = \left(\phi^{2k}*\tilde{v}_i^{(k)}\right),\]
%	with $\phi^{k} = \mathcal{L}^{-1}\left(\exp(-kh_{\min}\sqrt{s^{2\nu}+\kappa\xi^2})\right)$.
%	Using the Lemma \ref{estimate10} we have:
%	\begin{equation}
%		\| w_i^{(k)}\|_{L^{\infty}(0,T;L^2(-\infty,\infty))}\leq
%		\exp\left(-\alpha k^{1/(1-\nu)}\right)\| v_i^{(k)}\|_{L^{\infty}(0,T;L^2(-\infty,\infty))},
%	\end{equation}
%	Using above relation we have the proof.	
%	\hfill\end{proof}
%
%
%
%
%

